Object-Centric Unsupervised Image Captioning

Image captioning is a longstanding problem in the field of computer vision and natural language processing. To date, researchers have produced impressive state-of-the-art performance in the age of deep learning. Most of these state-of-the-art, however, requires large volume of annotated image-caption pairs in order to train their models. When given an image dataset of interests, practitioner needs to annotate the caption for each image in the training set and this process needs to happen for each newly collected image dataset. In this paper, we explore the task of unsupervised image captioning which utilizes unpaired images and texts to train the model so that the texts can come from different sources than the images. A main school of research on this topic that has been shown to be effective is to construct pairs from the images and texts in the training set according to their overlap of objects. Unlike in the supervised setting, these constructed pairings are however not guaranteed to have fully overlapping set of objects. Our work in this paper overcomes this by harvesting objects corresponding to a given sentence from the training set, even if they don't belong to the same image. When used as input to a transformer, such mixture of objects enables larger if not full object coverage, and when supervised by the corresponding sentence, produced results that outperform current state of the art unsupervised methods by a significant margin. Building upon this finding, we further show that (1) additional information on relationship between objects and attributes of objects also helps in boosting performance; and (2) our method also extends well to non-English image captioning, which usually suffers from a scarcer level of annotations. Our findings are supported by strong empirical results. Our code is available at https://github.com/zihangm/obj-centric-unsup-caption.

==> 1.abstract.snl.tex <==
\begin{abstract}
   Training an image captioning model in an unsupervised manner without utilizing annotated image-sentence pairs is an important step towards tapping into a wider corpus of text and images.
   The biggest challenge is that in the supervised setting, the images and texts we use during training are well matches -- usually all objects mentioned in the sentence appear in the corresponding image and thus the model can learn the mapping from image to sentence smoothly. However, in unsupervised setting, this information is lost. A main school of research that has been shown to be effective is to construct pairs from the images and texts in the training dataset according to their overlap of objects, but the pairs are usually not well matches since there may not exist well matches pairs in the given datasets at all.
   %A main school of research that has been shown to be effective is to construct pairs from the images and texts from the training dataset according to their overlap of objects. However, the quality of such artificially constructed pairs can be very limited because there may not exist good pairs where the sentence well describes the corresponding image in the given image and text datasets at all. 
   To this end, we propose to synthesize images utilizing detected objects, compositing objects into an image to form a pair with a given sentence. As a result, the images and texts used during our training are well matched -- one image contains all objects that appear in the corresponding sentence, bridging the most important gap between supervised and unsupervised image captioning. Interestingly, our findings show that in spite of losing fine-grained information (e.g., facial characteristics of a person), incorporating the synthesized images to form pairs with the sentences during training out-performs current state of the art unsupervised methods by a significant margin. 
   Most previous works only consider object category information during training, while a sentence can also describe the relationships between objects and some attributes of the objects. We demonstrate that our method can also naturally utilize these modular information when they are available during training to synthesize a better image for a given sentence and this leads to better performance. We further shows that when extending to non-English texts which usually suffers from much scarcer level of annotated training data, our proposed method is still able to generate reasonable caption predictions.
   Our findings are supported by strong empirical results.
   
 %  We also present two findings built on top of our proposed method that will be of interest to researchers. One, we found that our method performs better when we add other pre-trained models, namely object relationship and attribute detectors, in addition to the object detector. This effect can be directly attributed to our synthesis procedure, which allows for flexibly utilizing all the given information to synthesize a better image for a given sentence. Second, when extending to non-english text, which suffers from a much scarcer level of annotated training data, our proposed method is able to synthesize images to form pairs with given sentences. Our findings are supported by strong empirical results.
\end{abstract}

==> 1.abstract.tex <==
\begin{abstract}
   Training an image captioning model without utilizing annotated image-sentence pairs is an important step towards wider application of image captioning techniques. In this paper, we decompose the visual information contained in an image region into several components and investigate the effect of each component. Based on our hypothesis that removing one certain component (the fine-grained visual information) from images does not significantly influence the model performance, we propose a novel approach for unsupervised image captioning that creates an image from scratch to form the pair with a given sentence and use these artificially constructed pairs to train the model. Experiments on various datasets show that our method outperforms state-of-the-art methods by a clear margin. Our proposed framework relies on a pre-trained object detector and naturally enables utilizing various  pre-trained models like the relationship detector, to further improve the performance. Furthermore, our method can be easily extended to do image captioning for different languages and in this paper we use Chinese and French as examples. To our best knowledge, we are the first to demonstrate unsupervised image captioning for different languages. We will make our code publicly available.
    \sernam{Comment using this command}
\end{abstract}

==> 2.intro.tex <==
\section{Introduction}
\label{sec:intro}

The developments in computer vision (CV) and natural language processing (NLP) communities began to have more and more overlapping recently, driven by the need for multi-modal modeling, and image captioning is a crucial piece at the intersection of CV and NLP. A sizable amount of efforts have been devoted into improving the models for image captioning, from the early use of Convolutional Neural Networks combined with Recurrent Neural Networks fed with the global image feature \cite{karpathy2015deep}, to various attention mechanisms \cite{xu2015show,anderson2018bottom} and transformer based models \cite{cornia2020meshed}. The performance of image captioning has been greatly improved by these advances in recent years.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\columnwidth]{figs/intro_fig.pdf}
    \caption{Illustration of our constructed image.}
    \label{fig:tmp1}
\end{figure}

However, most of the works require paired image-sentence data, which is quite expensive to obtain. For example, in \cite{pont2020connecting} it costs 144.7 seconds on average for a professional full-time annotator to annotate a comprehensive caption of one single image. On the other hand, collecting an image dataset and a text dataset which are independent of each other is much cheaper, and there are plenty of existing image and text datsets. Thus how to utilize these unpaired data to train an image captioning model become crucial, especially considering that the scale of modern deep models and datasets grows very 
fast over time.

Some previous efforts have been devoted into this direction. \cite{feng2019unsupervised} made the first attempt on unsupervised image captioning by utilizing policy gradient to encourage the predicted caption to contain some visual concept. This supervision only encourages the appearance of visual object words, but is ignorant of how these visual object words fit in the sentence. Thus the performance is limited. Later work \cite{laina2019towards} proposed to mine pseudo image-sentence pairs to train the model and demonstrated its value: Given a sentence, it searches for an image in the existing dataset which has large visual concept overlapping with this sentence to form a pair. \cite{honda2021removing} proposed to improve the pseudo image-sentence pair approach by introducing a new gate function telling the model which word in the sentence is irrelevant to the image, but the training is still based on pseudo image-sentence pairs. One fundamental limitation of the previous approaches is that: Since in unsupervised image captioning task, the image dataset is independent with the text dataset, it is highly likely that there does not exist image-sentence pairs with large overlapping of visual concepts in the datasets. Thus mining pseudo image-sentence pairs could provide bad training data. 



In our paper, we try to solve the unsupervised image captioning task from a different perspective. Since the biggest challenge of unsupervised image captioning is that we may not have good image-sentence pairs in the given dataset, the question we try to explore is: Given a randomly chosen sentence, instead of trying to find an image from the existing dataset, can we artificially construct a novel image which forms a reasonable pair with this sentence? After carefully decomposing the visual information contained in an image into several components and analyzing the effect of the individual component, we find that this approach to construct the novel image (as illustrated in Fig. \ref{fig:tmp1}) is promising and has the potential of nearly matching the performance of supervised image captioning model. Given a sentence, we propose to construct a novel image using image regions mined from multiple existing images where each image region captures an object of some category, such that the constructed image covers all visual concepts detected from the sentence. 
Experiments show that our approach outperforms the state-of-the-art methods by a clear margin. 
 

In the setup described above, we follow previous works to assume a pre-trained object detector to be available. It will lead to an issue that the location of objects in the artificially constructed novel image does not necessarily reflect the relationship between different objects (e.g., the phrase ``person riding a bike'' requires the ``person'' to be above ``bike''). However, when a relationship detector also becomes available, our approach naturally enables the utilization of such relationship information by considering such information when constructing the novel images and it leads to further performance improvement. Most previous works \cite{feng2019unsupervised,laina2019towards,honda2021removing,guo2020recurrent} cannot easily enable the utilization of such relationship information without making significant change to their model or training procedure.

Moreover, we explore the possibility to go beyond English to generate captions in other languages while still assuming the same English-based object detector as it is easily enabled by our method. To our best knowledge, our work is the first one which demonstrated the ability to generate captions for different languages without the use of any paired information.

% Moreover, our experiments provide new insights on what is needed when training an image captioning model: When training a computer vision model that needs to perform some kind of inference for a given natural image during the test time, using
%To appreciate why this is nontrivial, consider any computer vision model that takes the natural images as input, if we replace the natural image with an image constructed using random chosen pieces from several different images, it feels intuitively that it would fail. But as shown by our experiments, this approach works well and outperform SOTA methods by a large margin.




To summarize our contribution:
\begin{itemize}
    \item We propose a novel approach to generate image-sentence pairs to train the model without utilizing any paired information. Given a sentence, we construct a novel image to form a pair with this sentence.
    \item Our approach naturally enables the use of various information provided through pre-trained models (not limited to object detector).
    % While previous methods are limited to searching within existing images in the given image dataset, so when there do not exist good image-sentence pairs, pretrained models cannot help.
    \item We are the first to demonstrate training image captioning models for different target languages without using any paired information.
\end{itemize}


==> 5.experiment.tex <==
\section{Experiments}
In this section, we first verify that utilizing object regions from different images together can lead to reasonable performance, even close to the supervised image captioning performance, by carefully designed experiments 
using images from COCO \cite{lin2014microsoft} and corresponding captions provided by Localized Narratives \cite{pont2020connecting}. 
Then we report results on independent image and caption sources and compare with baseline methods \cite{feng2019unsupervised,honda2021removing}. The image dataset we choose is COCO, and we conduct experiments using Google Conceptual Captions (GCC) \cite{sharma2018conceptual} and Shuttle Stocks  (SS) \cite{feng2019unsupervised} as the caption dataset respectively. Next we demonstrate how our framework can utilize relationship detector when it becomes available using COCO images and Localized Narratives captions on Open Images \cite{kuznetsova2020open}. Finally we show that our method can be easily adapted to train on other (non-English) languages by showing results on Chinese and French/Germany caption datasets.
 
\textbf{Evaluation Datasets.}
For images, we follow previous work \cite{feng2019unsupervised,honda2021removing} to use the MS COCO dataset and the train/validation/test split provided by \cite{karpathy2015deep}, and report the performance on the test split (except in Sec. \ref{sec:verify_hyp}, where we follow \cite{meng2021connecting} to use COCO-2017 official splits). For the text, we choose the recently released Localized Narratives (LN) \cite{pont2020connecting} which provides  captions for four public datasets including COCO, ADE20k, Flickr30k and Open Images. We choose LN-COCO instead of COCO captions \cite{chen2015microsoft} because the captions in LN are longer, contain more verbs, and the overall quality is also good 
(see our supplement or Table 2 in \cite{pont2020connecting} for a comparison between LN-COCO and COCO captions)
. We use LN-COCO for evaluation for all experiments except experiments on non-English languages in Sec \ref{sec:non-eng}, where we use the annotations provided by COCO-CN \cite{li2019coco} and Multi30k \cite{elliott2016multi30k}.


\begin{table*}[!ht]
    \centering
    % \small
    % \setlength{\tabcolsep}{4pt}
    % \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{l | c c c c c c c }
        \thickhline
        Methods & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & WMD \\
        \hline 
        Supervised training  & 0.306 & 0.082 & 0.151 & 0.306 & 0.263 & 0.238 & 0.113 \\
        After replacing objects & 0.297 & 0.078 & 0.145 & 0.298 & 0.227 & 0.232 & 0.109 \\
        After replacing objects and location & 0.298 & 0.080 & 0.146 & 0.300 & 0.239 & 0.234 & 0.108 \\
        \thickhline
    \end{tabular}
    % }
    \caption{The performance of supervised training, before and after replacing the objects with randomly mined objects of the same category (the supervised training was conducted following \cite{meng2021connecting} using their provided code). We can see that after the operation of replacing objects, the performance stays comparable. Detailed interpretation of each row is in Sec. \ref{sec:GCC_SS}.}
    \label{tab:verify_hyp1}
\end{table*}

% table
\begin{table*}[!h]
    \centering
    % \small
    % \setlength{\tabcolsep}{4pt}
    % \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{l l | c c c c c c c }
        \thickhline
        Text dataset & Method & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & WMD \\
        \hline 
        SS & \cite{feng2019unsupervised} & 0.016 & 0.001 & 0.037 & 0.109 & 0.018 & 0.073 & 0.045 \\
        SS & \cite{honda2021removing} & 0.022 & 0.001 & 0.043 & 0.126 & 0.025 & 0.078 & 0.042 \\
        SS & Ours & \textbf{0.056} & \textbf{0.003} & \textbf{0.060} & \textbf{0.127} & \textbf{0.038} & \textbf{0.102} & \textbf{0.060}\\
        \hline
        GCC & \cite{honda2021removing} & 0.006 & 0.000 & 0.035 & 0.115 & 0.017 & 0.075 & 0.040 \\
        GCC & Ours & \textbf{0.062} & \textbf{0.004} & \textbf{0.062} & \textbf{0.146} & \textbf{0.032} & \textbf{0.104} & \textbf{0.055} \\
        \thickhline
    \end{tabular}
    % }
    \caption{The performance of our method and baseline methods \cite{feng2019unsupervised,honda2021removing} trained using COCO images and SS/GCC text datasets, evaluated using test split of COCO images and LN-COCO caption annotations as ground truth. }
    \label{tab:gcc_ss}
\end{table*}

\textbf{Training Datasets.}
We use images from COCO training set in all of our experiments.
For experiments in Sec \ref{sec:verify_hyp}, we follow \cite{meng2021connecting} to use text from LN-COCO on the COCO-2017 train split; For comparing with baseline methods in Sec \ref{sec:GCC_SS} we conduct experiments on both Google conceptual Captions (GCC) \cite{sharma2018conceptual} and Shutterstock (SS) image description corpus provided by \cite{feng2019unsupervised}; For demonstrating the ability of our framework to utilize relationship information in Sec \ref{sec:exp_rel}, we train with captions from LN-OpenImages because the size is relatively large and the sentences contain rich relationship information. Finally for non-English languages in Sec \ref{sec:non-eng}, we use COCO-CN \cite{li2019coco} for Chinese language which provides Chinese captions for 20,342 images in COCO use the train/test split they provided.
We use Multi30k \cite{elliott2016multi30k} for French language which provides French captions for all of Flickr30k images and also 1k images from COCO. We used the captions on Flickr30k for training and the 1k image-caption pairs on COCO for evaluation. We exclude all the images contained in the train/val/test splits of COCO-CN/Multi30k from COCO train set when constructing the training image set to make sure there does not exist paired data in the training images and training text, and the test images remain unseen during training.




\textbf{Implementation Details.}
We first tokenize the text datasets and delete sentences which are shorter than $5$ words or longer than a certain length (20 for GCC and SS, 100 for Localized Narratives) and build a language vocabulary. Then we match the object words of the object detector with the language vocabulary. If the vocabulary is too large, we filter out the least frequently used words and set them to $\it{unk}$. Our object detector is a Faster R-CNN \cite{ren2015faster} pretrained on Visual Genome \cite{krishna2017visual}, whose vocabulary contains 1600 object words. The next step is to build a dictionary that maps an object word to a set of images which contain this object word. Finally, during training, for a randomly picked sentence, we first find all object words it contains, and for each object word, we randomly pick one image that contains this object word and crop this object region using its bounding box location. In this way, for each sentence we can have a set of object regions and we stitch them together to construct the new image $\hat{I}$. In Sec \ref{sec:exp_rel}, we additionally mine pairs of objects which have relationship and use them together with single objects when constructing the new image $\hat{I}$.

When working with non-English text datasets in Sec \ref{sec:non-eng}, we only need to translate each word in the  vocabulary of the object detector (English based) into the target language (while translating a whole sentence into different languages is generally hard, translating a single word is often easy and precise), and the rest procedure remains the same as that on English datasets.



\textbf{Experimental Settings.}
Our captioning model is a one layer transformer \cite{vaswani2017attention}. The hidden size of attention layers is 512 and that of the feed-forward layers is 2048. The input object features are extracted by the Faster R-CNN mentioned above. We train the network with batch size $30$ using the Adam optimizer \cite{kingma2014adam}. The initial learning rate is 5e-4, which decays by 0.8 every 3 epochs, for a total of 30 epochs. The same training setup is used for all experiments in this paper. 

\textbf{Baselines.}
In Sec \ref{sec:GCC_SS} we compare with previous works \cite{feng2019unsupervised,honda2021removing} using COCO images with GCC and SS as the text datasets respectively. We use the code released by the authors to reproduce their results for evaluation. Our work assumes the presence of a pretrained object detector, and the previous works \cite{feng2019unsupervised,honda2021removing} also assume a pretrained object detector but they do not utilize the bounding boxes. Thus we construct a baseline which follows \cite{honda2021removing,laina2019towards} to match a sentence to an existing image which has some overlapping with this sentence and train on these mined image-sentence pairs (see our supplement for more details), while keeping all other settings of our model (the same transformer, training parameters, and also utilizing object bounding boxes). This baseline also serves as an ablation study that allows us to directly compare our approach (mining a set of object regions $R_i$ for a given $S_i$) with the previous approach (searching for an existing image $I_j$ to form a pair with the given $S_i$).

\textbf{Evaluating Metrics.} 
We use the official COCO caption evaluation tool and report the performance in terms of BLEU-1 \cite{papineni2002bleu}, BLEU-4, METEOR \cite{banerjee2005meteor}, ROUGE \cite{lin2004rouge}, CIDEr \cite{vedantam2015cider}, SPICE \cite{anderson2016spice} and WMD \cite{kusner2015word}.

%preprocess image
%preprocess text
%build obj-text pairs
% relationship
% chinese

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/COCO-_SS_2.pdf}
    \caption{Qualitative results of our method and two baseline methods on COCO test split. ({\color{red} citation number [4] in the figure needs to be fixed in the end})}
    \label{fig:coco_ss}
\end{figure*}


\begin{table*}[!h]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    % \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{l l | c c c c c c c c }
        \thickhline
        Text dataset & Method & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & WMD & Object Coverage \\
        \hline 
        SS & Ours & \textbf{0.058} & \textbf{0.003} & \textbf{0.060} & \textbf{0.126} & \textbf{0.039} & \textbf{0.102} & \textbf{0.060} & \textbf{100\%}\\
        SS & Ours-half-obj & 0.056 & 0.002 & 0.055 & 0.117 & 0.036 & 0.082 & 0.055 & 50.0\% \\
        SS & Ours-baseline1 & 0.040 & 0.002 & 0.045 & 0.104 & 0.021 & 0.068 & 0.049 & 57.4\% \\
        \hline
        GCC & Ours  & \textbf{0.062} & \textbf{0.004} & \textbf{0.062} & \textbf{0.146} & \textbf{0.032} & \textbf{0.104} & \textbf{0.055} & \textbf{100\%} \\
        GCC & Ours-half-obj & 0.057 & 0.003 & 0.054 & 0.140 & 0.025 & 0.080 & 0.050 & 50.0\% \\
        GCC & Ours-baseline1 & 0.046 & 0.002 & 0.048 & 0.131 & 0.025 & 0.073 & 0.047 & 68.8\% \\
        \thickhline
    \end{tabular}
    % }
    \caption{Ablation study of our method. Baseline1 is the model trained with pseudo $(I_i,S_i)$ pairs (defined in Sec. \ref{sec:GCC_SS}). Object Coverage refers to the ratio that for a given sentence, how many percent of the objects in this sentence appears in the corresponding image used during training, averaged over all used training pairs. Our method has 100\% object coverage by construction since our synthesized image will contain all objects in the given sentence (here we only consider those object categories which can be detected by the pre-trained object detector).}
    \label{tab:gcc_ss_ablation}
\end{table*}

\subsection{Verify the effects of utilizing objects from different images}
\label{sec:verify_hyp}
To empirically verify the effects of utilizing object regions from different images, we start from standard supervised image captioning training, where we use the same transformer model and experimental settings as \cite{meng2021connecting} (\cite{meng2021connecting} utilizes trace information in addition to caption and images and we deleted the head for trace in their model) by  utilizing their provided code.
We use COCO images and LN-COCO to train a captioning model and its performance is in the {\it first row} of Table \ref{tab:verify_hyp1}. Then for each image-sentence pair in the training set, we detect all object regions in the image and replace each object region with another one of the same category mined from other images in the dataset and extract visual features from these mined regions before feeding into the transformer model. When we concatenate the 5-D location vector of a bounding box with its visual feature, we use its original location in the paired image.
Its performance is in the {\it second row} of Table \ref{tab:verify_hyp1}. Then we tried replacing the object region and also replace the 5-D location vector with that of the object region mined from other images. The result is in the {\it third row} of Table \ref{tab:verify_hyp1}.

We can see that after replacing the object regions with randomly picked objects of the same category, the performance does not have significant drop, which empirically shows that our proposal to use object regions from different images together is valid. We can also tell by comparing  the second and third rows that after replacing the objects, the location of the bounding box does not have  much influence.


% table
\begin{table*}[!h]
    \centering
    % \small
    % \setlength{\tabcolsep}{4pt}
    % \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{l | c c c c c c c }
        \thickhline
        Pretrained models & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & WMD \\
        \hline 
        object  & 0.327 & 0.059 & 0.140 & 0.262 & 0.109 & 0.181 & 0.079 \\
        object + attribute & \textbf{0.332} & 0.059 & 0.136 & 0.266 & 0.124 & 0.181 & 0.079\\
        object + relationship  & 0.329 & 0.061 & 0.140 & 0.268 & 0.120 & 0.188 & 0.080 \\
        object + relationship + attribute & 0.329 & \textbf{0.062} & \textbf{0.141} & \textbf{0.274} & \textbf{0.138} & \textbf{0.193} & \textbf{0.083}\\
        \thickhline
    \end{tabular}
    % }
    \caption{The performance of utilizing only object detector and that of utilizing object detector plus relationship detector. The models are trained using COCO images and LN-OpenImages captions, and evaluated using the test split of COCO images and LN-COCO caption annotations as ground truth.}
    \label{tab:rel}
\end{table*}

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/COCO-_Chinese.pdf}
    \caption{Qualitative results of our method trained on COCO images and COCO-CN (Chinese) sentences. Images associated with sentences from COCO-CN are deleted from the training image set such that no training sentence is associated with a training image.}
    \label{fig:coco_chinese}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/COCO-_French.pdf}
    \caption{Qualitative results of our method trained on COCO images and Multi30k (French) sentences.}
    \label{fig:coco_french}
\end{figure*}

\begin{table*}[!h]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l l l | c c c c c c c }
        \thickhline
        Training  text & Test text & Method & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & WMD \\
        COCO-CN (Chinese) & COCO-CN (Chinese) & Ours & \textbf{0.256} & \textbf{0.039} & \textbf{0.121} & \textbf{0.228} & \textbf{0.349} & \textbf{0.117} & \textbf{0.272} \\
        Multi30k(English) & COCO-CN (Chinese) & Baseline-translate & 0.005 & 0.000 & 0.072 & 0.086 & 0.002 & 0.095 & 0.000 \\
        COCO-CN (Chinese) & COCO-CN (Chinese) & Baseline-existing & 0.176 & 0.020 & 0.119 & 0.189 & 0.198 & 0.047 & 0.259 \\
        \hline
        Multi30k (French) & Multi30k (French) & Ours & \textbf{0.174} & \textbf{0.010} & \textbf{0.094} & \textbf{0.173} & \textbf{0.120} & \textbf{0.014} & \textbf{0.079} \\
        Multi30k (English) & Multi30k (French) & Baseline-translate & 0.104 & 0.000 & 0.053 & 0.092 & 0.099 & 0.006 & 0.056\\
        Multi30k (French) & Multi30k (French) & Baseline-existing & 0.126 & 0.008 & 0.086 & 0.154 & 0.059 & 0.013 & 0.078\\
        
        \thickhline
    \end{tabular}
    }
    \caption{Quantitative results of our method on COCO images and two text datasets of different languages (Chinese and French). ``Baseline-translate'' is defined in Sec. \ref{sec:non-eng}.}
    \label{tab:chinese}
\end{table*}


\subsection{Compare With State-of-the-Art Methods on GCC and SS Caption Datasets}
\label{sec:GCC_SS}
The task of unsupervised image captioning remains underexplored in recent years. We compare with \cite{feng2019unsupervised,honda2021removing} on COCO images with GCC sentences and SS sentences respectively. The quantitative results are in Fig. \ref{tab:gcc_ss}. We can see that our method outperforms all baseline methods on two text datasets by a clear margin. The qualitative results are in Table. \ref{fig:coco_ss}. The captions generated by  \cite{feng2019unsupervised} usually contains verbs describing the objects but make mistakes frequently (e.g., in ``a person is sitting on a motorbike'' the verb ``sitting'' matches with object ``motorbike'' but does not match the input image); \cite{honda2021removing} generates mostly correct captions but the captions are mainly concatenations of object names (nouns) without verbs describing the action of the object or the relationship between objects (e.g., ``a young man in a white skies''); Our method generates more comprehensive captions with mostly correct nouns and verbs and the captions are aware of the interaction between objects for most part (e.g., ``female skier wearing red jacket'', ``standing with skis on snow mountain slope''). 

We can also see that all methods fail to identify the color, and this is a limitation of only having a pre-trained object detector with no color attribute detector. If a pre-trained color detector becomes available, our method naturally enable the utilization of this information as described in Sec. \ref{sec:utilize_more_info}.

\textbf{Ablation Study.}
Note that although \cite{feng2019unsupervised,honda2021removing} and our method all assume a pre-trained object detector, \cite{feng2019unsupervised,honda2021removing} only utilize the category but not the bounding box of the detected object. On the other hand, we utilize both category and bounding box of the detected object. To demonstrate the benefit of our approach more clearly, we construct a baseline method (we call it ``ours-baseline1'') which shares all experimental settings with our method but instead of constructing $(R_i,S_i)$ pairs, it follows \cite{laina2019towards,honda2021removing} to mine pseudo pairs $(I_i,S_i)$ from existing image and text datasets. The results are in Table \ref{tab:gcc_ss_ablation}. We can see that by mining pseudo pairs performs significantly worse than our method, which demonstrates the benefit of constructing $(R_i,S_i)$ pairs for training. To further show that our method produces high quality training pairs, we compare the object coverage between our method and mining pairs from existing images and texts, shown in Table \ref{tab:gcc_ss_ablation}. The object coverage here is defined as: for a given sentence, how many percent of the object words in the sentence appear in the corresponding image which is used during training. For supervised image captioning, the object coverage is usually 100\%, which means that all objects in the sentence will appear in the pairing image. Our method also have 100\% object coverage and this is ensured by construction using our image synthesis procedure, while if we mine pairs from existing images and texts, there will be at least one third of the objects in the sentence not appearing in the corresponding images, which shows that these images and texts don't match well. We in addition conduct experiments by artificially dropping half of the object coverage from our approach and conduct the training (denoted as "Ours-half-obj" in Table \ref{tab:gcc_ss_ablation}), we can see that this has negative influence on the performance.


\subsection{Utilizing Relationship and Attribute Information}
\label{sec:exp_rel}

In Sec. \ref{sec:utilize_more_info} we described how our framework  naturally enables utilizing more pre-trained models when they become available to further improve the performance. Here we take the relationship detector as an example. We use the relationship detector and attribute detector pre-trained on Visual Genome (provided by \cite{zellers2018neural}) for images and the semantic parser provided by \cite{anderson2016spice} which is built on \cite{schuster2015generating} to find relationship triplets from sentences. Note that we only need the pre-trained relationship detectors during training to construct $(R_i,S_i)$ pairs, not test time. We train the model on COCO images, and choose LN-OpenImages as the text dataset since it contains rich semantic relationship information. Ideally when the subject-relation-object in the triplet completely match another triplet we say that these two triplets match.  But we find that very few triplets from the images can fully match the triplets from the sentences because of the noise of relationship detectors and the discrepancy between the image relationship detector and the sentence relationship detector. Thus in the experiment we do a vague matching: as long as the subject-object pair matches between two triplets, we process these two triplets as matched. The quantitative results are in Table \ref{tab:rel}, where we can see that adding relationship detector and attribute detector respectively both boost the performance compared with using object detector alone. We also see that adding both relationship and attribute detectors at the same time performs similarly to only adding relationship detector, while the relationship detector shows to be more beneficial than the attribute detector.
The qualitative results of our model utilizing object and relationship detectors are in Fig. \ref{fig:coco_ss} (the last row). We can see that the captions are  comprehensive and contain many relationship triplets in the generated captions (e.g., ``he-holding-ski sticks'', ``he-wearing-helmet'', ``man-standing on-land'').




\subsection{Unsupervised Captioning for Non-English Languages}
\label{sec:non-eng}

In this section we show the results of extending our method to train image captioning model for non-English languages. We choose Chinese and French as examples because of their wide use. To our best knowledge, our work is the first to show experiments on unsupervised image captioning for multiple languages and we do not have previous methods to directly compare with. Here we construct a baseline by using our method to train on COCO images and multi30k-English sentences , and then use Google Translate to translate the generated English captions into Chinese and French, respectively, to compare with our method which is directly trained on Chinese/French. We call this baseline ``Baseline-translate''.
The quantitative results are in Table \ref{tab:chinese}. We can see that our method directly train on the target language performs better than our constructed ``baseline-translate'' that trains on English and then translate the captions into the target language, which demonstrates the benefits of our approach that enables directly training on the target language in the unsupervised way. The qualitative results are in Fig. \ref{fig:coco_chinese} (Chinese) and Fig. \ref{fig:coco_french} (French). 

%during the word translation some loss of info. 



==> method_bak.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/overall_arch_v2.pdf}
    \caption{Overview of our unsupervised image captioning training pipeline. During training, the transformer takes the constructed image as input. During test/inference, it takes the natural image as input.}
    \label{fig:overall_arch}
\end{figure*}

\section{Method}
Given a set of images $\mathcal{I}=\{I_1,..., I_{N_i}\}$, and a set of sentences $\mathcal{S}=\{S_1,..., S_{N_s}\}$, our goal is to train a model which takes an image as input and generates a caption that well describes the input image. We follow previous work on unsupervised image captioning \cite{feng2019unsupervised} in assuming that we do not have information about the pairing between $\mathcal{I}$ and $\mathcal{S}$, but have access to a pretrained object detector. Our overall approach is shown in Fig. \ref{fig:overall_arch}, where we propose to mine objects from $\mathcal{I}$ without the constraint that these objects need to come from the same image. We first introduce our motivation and the key hypothesis in Sec. \ref{sec:motivation}. Next we describe how training pairs are formed with given sentences in Sec. \ref{sec:construct_new_img}, and then demonstrate how this approach naturally enables the utilization of additional knowledge when it becomes available in Sec. \ref{sec:utilize_more_info}. Finally we show how we extend to different languages with the same English-based object detector in Sec. \ref{sec:method_non_english}.

\subsection{Create a Novel Image to Match a Sentence}
\label{sec:construct_new_img}
In the previous section we start from the supervised setting and replace each object region with another one of the same category mined from other images in the dataset. In this section we need to do this operation from the opposite direction: Given a sentence $S_i$, we start from scratch and gradually add the image region mined from the dataset of the category specified by the sentence $S_i$, ending up with a created image $\hat{I_i}$ whose category visual information matches well with $S_i$.

Our approach is described as follows: Given a sentence $S_i$, we first detect the set of visual concepts it contains (e.g., person, bike),
\begin{equation}
    \mathcal{V}^S_i = \{v_1, v_2, ..., v_k\}
\end{equation}
where $k$ is the number of visual concepts in the sentence $S_i$, and then we use them to mine a set of image regions
\begin{equation}
\label{eq:img_region_objs}
    \mathcal{R}_i = \{r_1,r_2,...,r_k\}
\end{equation}
where each image region $r_j\in \mathcal{R}_i$ is from a randomly chosen image $I \in \mathcal{I}$ which contains the object of visual concept $v_j\in \mathcal{V}^S_i$.

Finally we paste all image regions in $\mathcal{R}_i$ together to construct the new image $\hat{I_i}$. When putting these image regions together, we keep their height, width and location in the original images where they are mined from since we did not have information about their size from the sentence.
\begin{equation}
    \hat{I_i} = \text{stitch }\mathcal{R}_i\text{ together}
\end{equation}

$\hat{I_i}$ forms a pair with the given sentence $S_i$. Then we can utilize these artificially constructed $\hat{I}$--$S$ pairs to train the captioning model using Cross Entropy (CE) loss,
\begin{equation}
    L = \text{CE}(f(\hat{I_i}), S_i)
\end{equation}
where $f$ represents the captioning model which maps an image into a sentence.
In our work, we utilize a transformer model \cite{vaswani2017attention} as the captioning model (we refer readers to \cite{vaswani2017attention} for more details about the architecture of the transformer model). Previous works \cite{anderson2018bottom,changpinyo2019decoupled,pont2020connecting} which use the transformer model for image captioning first utilize an object detector to extract multiple image regions and use these image regions as input tokens to the transformer model. In our work, since our $\hat{I_i}$ is constructed from the set of image regions $\mathcal{R}_i$, we can directly use $\mathcal{R}_i$ as the input tokens.

\subsection{Utilizing Other Pre-trained Models Beyond the Object Detector}
\label{sec:utilize_more_info}
When we construct $\hat{I_i}$ for a given $S_i$ using the approach described in Sec. \ref{sec:construct_new_img}, $\hat{I_i}$ will match  category information and a part of location information contained in $S_i$, but a large part of location information and fine-grained visual information in $\hat{I_i}$  may not match $S_i$, which could lead to some errors in $\hat{I_i}$ like wrong interactions between image regions or wrong scene, etc. Note that this is a limitation of only having an object detector, but not a limitation of our proposed method to construct $\hat{I_i}$. If other pre-trained models become available at training time, our method naturally enables utilizing them. In this section we take the pre-trained relationship detector and attribute detector as examples, and similar strategy could be adapted to other pre-trained models like scene detector, facial expression detector, etc.

We assume that for a given $I_i$, the relationship detector  can detect triplets in the form of subject-relation-object,
\begin{equation}
    \mathcal{T}^I_i = \{\text{sub}_1\text{-rel}_1\text{-obj}_1, ..., \text{sub}_{N_i^I}\text{-rel}_{N_i^I}\text{-obj}_{N_i^I}\}
\end{equation}
and for a sentence $S_i$, the relationship parser can detect triplets in the same form,
\begin{equation}
    \mathcal{T}^S_i = \{\text{sub}_1\text{-rel}_1\text{-obj}_1, ..., \text{sub}_{N_i^S}\text{-rel}_{N_i^S}\text{-obj}_{N_i^S}\}
\end{equation}
Then for a given sentence $S_i$, again we construct the set of image regions $\mathcal{R}_i$ using the same strategy as that in \eqref{eq:img_region_objs}. However, instead of only containing image regions which match the visual concepts in $S_i$, $\mathcal{R}_i$ here also contains  pairs of image regions (sub-obj) which match the triplets (sub-rel-obj) in $\mathcal{T}^S_i$:
\begin{equation}
    \mathcal{R}_i = \{r_1, ..., r_k, pair_1, ..., pair_l\}
\end{equation}
where each $r$ refers to one image region and each $pair$ refers to a pair of image regions formed by the subject region and the object region from one triplet. $k$ is the number of visual concepts in $S_i$ and $l$ is the number of triplets in $S_i$ detected by the language relationship detector. The following steps for construct training pairs and conduct training are the same as that in Sec. \ref{sec:construct_new_img}.

To utilize the pre-trained attribute detector, the steps are the same as that for utilizing the relationship detector. The only difference is that instead of detecting triplets subject-relation-object, the attribute detector detects pairs in the form of attribute-object. Then when we see a certain attribute-object pair in the sentence $S_i$, we can look for an image region that matches this attribute-object, and add this image region into $\mathcal{R}_i$.

\subsection{Limits of Unsupervised Image Captioning}
\label{sec:motivation}

\textbf{Decompose the Visual Information of an Image Region.}
%\zihang{First divide the information into several parts, such that replacing an object discard one of them... this way feels better to explain, and can also point out our limitation clearly (what info do we lose by replacing an object)}
We start by considering this question: given a sentence $S$, how do we find an image which matches with this sentence? 
To answer this, we divide the visual information contained in an image region (e.g., the bounding box region of an object in an image) into three components: \begin{enumerate*}[label=(\roman*)] \item object category information (which category/categories does the object belong to), \item object location information (where is the object located in the image) and \item fine-grained object information (the visual information of the object beyond the object category) \end{enumerate*}. Taking the image region which contains a ``man'' in Fig. \ref{fig:overall_arch} for example, the object category is ``person'' or ``man'', the location is described by its bounding box location, and the fine-grained information could contain the facial features of this person and his action. These components together will further determine the relationship between this object and other objects. For example, if we have ``person riding a bike'' in the image, we would expect to see the ``person'' located closely above the ``bike'', and the action of ``person'' also corresponds to ``ride''. In an image-sentence pair, all these three components of the image need to match with the semantics of the sentence. 

\textbf{Exploring the Effect of Fine-grained Object Information.}
Now consider our unsupservised captioning task, the information we can get from an image is given by the assumed pre-trained object detector, which gives us the object category information and a part of the object location information, but no fine-grained visual information. If the fine-grained visual information is crucial for the performance when training an image captioning model, then our considered unsupervised captioning task will be fundamentally limited by the absence of this information. However, based on the observation that most sentences in the commonly used captioning datasets do not contain much fine-grained information (like facial features of a person or exact shape of an umbrella), we make the following hypothesis which motivates our approach, 

\begin{hyp} 
\label{hyp:1}
For the purpose of training an image captioning model, removing the fine-grained visual information from the images in image-sentence pairs during training does not greatly influence the model.
%given an image-sentence pair, if we replace one object in the image with an object of the same category from another image in the image dataset, the training performance is approximately the same. 
%In other words, the visual information shared across the same category is far more important than the information .
% For the purpose of training an image captioning model, the information in an image is mostly captured by the category of objects and the interactions reflected from their spatial locations. For an image-sentence pair, if we replace one object in the image with an object of the same category from another image in the image dataset, the training performance is approximately the same.
\end{hyp}

\textbf{Verifying Hypothesis \ref{hyp:1}.}
We then carefully design experiments to empirically verify this hypothesis. We start from the standard supervised image captioning setting, where we have access to paired image-sentence pairs during training. Then for each image-sentence pair in the training set, we detect all object regions in the image and replace each object region with another one of the same category mined from other images in the dataset. Note that this operation is designed to keep the category visual information and location information, but remove the fine-grained object information (e.g., a ``person'' may be replaced with a different person with a different action/gesture, as shown in Fig. \ref{fig:overall_arch}). The results show that after performing this operation during training, the performance of the trained image captioning model only has marginal drop, which indicates the validness of our hypothesis \ref{hyp:1}. The details of this experiment are in Sec. \ref{sec:verify_hyp}.

\textbf{The Implication of Hypothesis \ref{hyp:1}: the Limit of Unsupervised Image Captioning.}
Note that the above hypothesis being true suggests where the limit of unsupervised image captioning (while only assuming a pre-trained object detector) is: 
The best performance an unsupervised image captioning model can possibly get is exactly the performance of the model which is trained in a supervised fashion but with the fine-grained visual information removed, since in both ways the information we have during training is the category visual information and location information.
Then hypothesis \ref{hyp:1} being true informs that the best possible performance of an unsupervised model can indeed be very close to that of a supervised model.

% The main concept of hypothesis \ref{hyp:1} is demonstrated in Fig X, where XXXX. In our experiment section, we empirically verify that our hypothesis \ref{hyp:1} holds. 
 
The fact that hypothesis \ref{hyp:1} holds also motivates our approach: for a given sentence $S$, it is possible to create a new image from scratch by choosing proper image regions from the given image dataset which match the category information and location information (to the extent possible) of $S$. 
%\zihang{This transition part feels a little unclear. I'm still thinking of how to improve } 







\subsection{Extension to Other Languages}
\label{sec:method_non_english}
Most current works on image captioning are based on English, as well as the works on object detection. In this section we show that we can easily adapt our work to train an image captioning model for different target languages other than English in a unsupervised way. We still  assume the same pre-trained object detector trained on English vocabulary.  We denote the English vocabulary of the object detector as,
\begin{equation}
    \text{voc}_\text{English} = \{\text{word}_1, ..., \text{word}_{N_\text{English}}\}
\end{equation}
Then we translate each word in the English vocabulary into the target language denoted as ``Target'' (although translating a whole sentence into a different language is a challenging task, translating a single word can be easily done using language dictionaries), 
\begin{equation}
    \text{voc}_\text{Target} = \{\text{word}_1, ..., \text{word}_{N_\text{Target}}\}
\end{equation}
where $N_\text{English}$ may not equal to $N_\text{Target}$ considering it is possible that multiple words in English are translated into the same word in the target language.
After this, we can follow the same steps in Sec. \ref{sec:construct_new_img} to construct $(\hat{I_i}, S_i)$ pairs to train a model directly in the target language.




